LEAGUE: Guided Skill Learning and Abstraction for Long-Horizon Manipulation

To assist with everyday human activities, robots must solve complex long-horizon tasks and generalize to new settings. Recent deep reinforcement learning (RL) methods show promise in fully autonomous learning, but they struggle to reach long-term goals in large environments. On the other hand, Task and Motion Planning (TAMP) approaches excel at solving and generalizing across long-horizon tasks, thanks to their powerful state and action abstractions. But they assume predefined skill sets, which limits their real-world applications. In this work, we combine the benefits of these two paradigms and propose an integrated task planning and skill learning framework named LEAGUE (Learning and Abstraction with Guidance). LEAGUE leverages the symbolic interface of a task planner to guide RL-based skill learning and creates abstract state space to enable skill reuse. More importantly, LEAGUE learns manipulation skills in-situ of the task planning system, continuously growing its capability and the set of tasks that it can solve. We evaluate LEAGUE on four challenging simulated task domains and show that LEAGUE outperforms baselines by large margins. We also show that the learned skills can be reused to accelerate learning in new tasks domains and transfer to a physical robot platform.

==> text/alg_singleline.tex <==
\begin{wrapfigure}[10]{R}{0.5\textwidth}
    \begin{minipage}{\textwidth}
    \vspace{-.3in}
    \begin{algorithm}[H]
    	\footnotesize
        \caption{Skill Learning}\label{alg:sk_learn}
        \begin{algorithmic}[1]
            \State \textbf{hyperparameters:} \\
            Number of training iterations $K$
            \State \textbf{input:} \\
            \texttt{env}  \Comment{task environment} \\
            $g$  \Comment{symbolic task goal} \\
            $\Bar{\Psi}$ \Comment{state predicates} \\
            $\Bar\Omega$ \Comment{lifted operators}
            \State \textbf{start} \\
            $\Pi \leftarrow [\pi_{1}^{0}, ..., \pi_{N}^{0}]$ 
            \State // initialize all skill controllers \\
            $t \leftarrow 0$
            \While {\emph{Not Converged}}
            \State $\mathcal{D}\leftarrow \emptyset$
            \For{$i \leftarrow [1, ..., N]$}
            \State $\mathcal{D} \leftarrow \mathcal{D} \cup
            \textsc{PlanningWithSkills}(\texttt{env}, g, \Bar{\Psi}, \Bar\Omega, \Pi)$
            \EndFor
            \State // evaluate planner and collect failed skills
            \For{$i, s_i, \underline{\omega} \leftarrow \mathcal{D}$}
            \State $\pi_i^{t} \leftarrow \Pi[i]$
            \For{$k \leftarrow [1, ..., K]$}
            % \State \texttt{env.set_sim($s_i$)}  
            % \State // set simulator state
            \State $\pi_{i}^{t+k} \leftarrow\textsc{Optimize}(\texttt{env}, \pi_{i}^{t+k-1}, \underline{\omega})$
            \State // RL training
            \EndFor
            \State $\Pi[i] \leftarrow \pi_{i}^{t+K}$
            \EndFor
            \State $t \leftarrow t+K$
            \EndWhile
            \State \Return $\Pi$
        \end{algorithmic}
    \end{algorithm}
    \end{minipage}
\end{wrapfigure}


==> text/pddl/HDDL.tex <==
% This file is part of https://github.com/Maumagnaguagno/Planning_LaTeX
\lstdefinelanguage{HDDL}
{
  sensitive=false,    % not case-sensitive
  morecomment=[l]{;}, % line comment
  alsoletter={:,-},   % consider extra characters
  morekeywords={
    define,domain,problem,not,and,or,forall,exists,
    :domain,:requirements,:typing,:hierarchy,:equality,:negative-preconditions,
    :method-preconditions,:universal-preconditions,:universal-effects,:existential-preconditions,
    :types,:predicates,:action,:parameters,:precondition,:effect,
    :task,:method,:subtasks,:tasks,:ordered-subtasks,:ordered-tasks,:ordering,:constraints,
    :htn,:init,:goal,:objects
  }
}

==> text/pddl/JSHOP.tex <==
% This file is part of https://github.com/Maumagnaguagno/Planning_LaTeX
\lstdefinelanguage{JSHOP}
{
  sensitive=false,    % not case-sensitive
  morecomment=[l]{;}, % line comment
  alsoletter={:,-},   % consider extra characters
  morekeywords={
    defdomain,defproblem,not,and,or,imply,forall,assign,call,nil,
    :first,:sort-by,:immediate,:unordered,:operator,:method,:protection,:-
  }
}

==> text/pddl/PDDL.tex <==
% This file is part of https://github.com/Maumagnaguagno/Planning_LaTeX
\lstdefinelanguage{PDDL}
{
  sensitive=false,    % not case-sensitive
  morecomment=[l]{;}, % line comment
  alsoletter={:,-},   % consider extra characters
  morekeywords={
    define,domain,problem,not,and,or,when,forall,exists,either,
    :domain,:requirements,:types,:objects,:constants,
    :predicates,:action,:parameters,:precondition,:effect,
    :fluents,:primary-effect,:side-effect,:init,:goal,
    :strips,:adl,:equality,:typing,:conditional-effects,
    :negative-preconditions,:disjunctive-preconditions,
    :existential-preconditions,:universal-preconditions,:quantified-preconditions,
    :functions,assign,increase,decrease,scale-up,scale-down,
    :metric,minimize,maximize,
    :durative-actions,:duration-inequalities,:continuous-effects,
    :durative-action,:duration,:condition
  }
}

==> text/related.tex <==
\section{Related Work}
\label{sec:related}


\noindent\textbf{TAMP and Learning for TAMP.} 
% TAMP overview
% Learn operators
% Learn predicates
% Learn samplers
Task and Motion Planning (TAMP)~\cite{kaelbling2011hierarchical,kaelbling2013integrated,garrett2020pddlstream,toussaintlogic,toussaint2018differentiable,garrett2020integrated} is a powerful paradigm to solve long-horizon manipulation tasks. The key idea is to break a challenging planning problem into a set of symbolic-continuous search problems that are individually easier to solve. However, TAMP methods require high-level skills and their kinematics or dynamics models \emph{a priori}. The assumptions preclude domains for which hand-engineering manipulation skills is difficult, such as contact-rich tasks. Recent works proposed to learn dynamics models for TAMP by characterizing skill preconditions and effects~\cite{kaelbling2017learning,curtis2022discovering,wang2018active,pasula2007learning,xia2018learning,konidaris2018skills,silver2022inventing,liang2022search}. For example, Konidaris {et al.}~\cite{konidaris2018skills} learns compact symbolic models of an environment through trial-and-error. Liang {et al.}~\cite{liang2022search} uses graph neural networks to model skill effects. However, these works still require hand-engineering complete skill sets that can solve the target task, which may not be feasible in real-world applications. Our idea of learning skills to augment TAMP systems is closely related to Silver {et al.}~\cite{silverlearning}, which proposed to learn neural-symbolic skills via imitation. But they require access to hard-coded demonstration policies that can readily solve the target tasks. Our work instead aims to progressively grow TAMP skill libraries via guided reinforcement learning to solve long-horizon contact-rich manipulation tasks. 
 
\noindent\textbf{Curriculum for RL.}
% curriculum RL, meta RL, multitask RL
% We utilize the 
Our idea to guide skill learning with a symbolic task planner is connected to the curriculum for RL. The key idea is to expose a learning agent to incrementally more difficult intermediate tasks before mastering a target task~\cite{narvekar2020curriculum}. The intermediate tasks can take the form of state initialization~\cite{florensa2017reverse,nair2018overcoming,fang2019curriculum}, environments~\cite{cobbe2020leveraging,fang2020adaptive,baker2019emergent}, and subgoals~\cite{sarathy2021spotter,campero2021learning,florensa2018automatic,narvekar2016source,sharma2021autonomous, uchendu2022jump}. For example, Florensa {et al.}~\cite{florensa2017reverse} and VaPRL~\cite{sharma2021autonomous} start with near-success initialization and gradually move the initial states further away. Campero {et al.}~\cite{campero2021learning} trains a goal-generator teacher and a goal-seeking student. While effective at accelerating task learning, existing curricula focus on teaching tasks or domain-specific policies. In contrast, our method leverages the symbolic abstraction of a task planner to learn a repertoire of modular and composable skills. We show that we can compose learned skills to achieve new goals and even transfer skills to new task domains. 
% Different from these approaches, we utilize a symbolic planner to decompose the task. The generated plan skeleton will sequence the learning of the skill policies, where the subgoal for each operator will serve as guidance for constructing the reward function, allowing us to gradually master skills in an efficient and modular way for accomplishing the final task goal. 

\noindent\textbf{State and Action Abstractions.}
% symbolic planning, contextural obs, task-related abstractions
State and action abstractions are crucial for learning complex tasks in a large environment~\cite{abel2022theory}. State abstraction allows agents to focus on task-relevant features of the environment. Action abstraction enables temporally-extended decision-making for long-horizon tasks. There exists a large body of work on learning either or both types of abstractions~\cite{sutton1999between,koller1999computing,jonschkowski2015learning,konidaris2018skills,zhang2020learning,abel2020value, chitnis2020camps, liang2022search, xu2021deep}. For example, Jonschkowski {et al.}~\cite{jonschkowski2015learning} explores different representation learning objectives for effective state abstraction. Abel {et al.}~\cite{abel2020value} introduces a theory for value-preserving state-action abstraction. However, autonomously discovering suitable abstractions remains an open challenge. Our key insight is that a TAMP framework provides powerful state and action abstractions that can readily guide skill learning. Specifically, the symbolic interface of an action operator defines both the precondition and the effect (action abstraction) and the state subspace that is relevant to the action (state abstraction). The abstractions allow us to train skills that are compatible with the task planner and prevent the learned skills from being distracted by irrelevant objects, making skill reuse across tasks and domains possible.

\noindent\textbf{Hierarchical Modeling in Robot Learning.}
% Hierarchical RL and PAMDP
% neural task programming
Our method inherits the bi-level hierarchy of a TAMP framework. Hierarchical modeling has a rich history in robotics and robot learning. In addition to TAMP, various general frameworks including hierarchical task networks~\cite{xu2019regression, wang2022generalizable, nejati2006learning,sohrabi2009htn,xu2018neural,huang2019neural}, logical-geometric programming~\cite{toussaintlogic,toussaint2018differentiable}, and hierarchical reinforcement learning (HRL)~\cite{nachum2018data,bacon2017option,vezhnevets2017feudal} have been proposed to exploit the hierarchical nature of common robotics tasks. In the context of HRL, a small number of works have explored symbolic planner-guided HRL~\cite{yang2018peorl,illanes2020symbolic}. However, these methods require tabular state representations and are thus limited to simple grid-world domains. In robotics domains, a closely related research thread is to use behavior primitives in RL~\cite{nasiriany2022maple,dalal2021accelerating}. For example, MAPLE~\cite{nasiriany2022maple} trains a high-level policy that chooses hand-engineered behavior primitives and atomic actions. Our method instead leverages a symbolic planner to serve as the high-level controller to compose learned skills, allowing us to continuously extend the skill set while also leading to better generalization.
